Triangulation of Points Constrained to a Plane

We study the set of image tuples arising from fixed cameras observing varying planar 3-dimensional point configurations. We derive a formula for the number of complex critical points of the triangulation problem, which seeks to reconstruct such configurations from noisy image data. Valid for an arbitrary number of views, this formula quantifies the intrinsic algebraic complexity of planar triangulation. We validate our theoretical findings through numerical experiments on both synthetic and real data, demonstrating that incorporating the planar incidence constraints leads to faster point reconstruction and improved accuracy compared to unconstrained triangulation.

==> figs/real_test_3v.tex <==
%\begin{tikzpicture}

\begin{axis}[%
xmode=log,
width=0.38\columnwidth,
height=0.25\columnwidth,
at={(2.2in,0.389in)},
scale only axis,
xmin=1e-4,
xmax=100,
xlabel style={font=\color{white!15!black}},
xtick={0.001,0.01,0.1,1,10},
xlabel={$\epsilon_{tr}$ (meters)},
%xtick={1e-15,1e-10,1e-5,1e-0},
title={Triangulation error $m=3$},
ymin=0,
ymax=400,
ymode=normal,
yminorticks=true,
%ytick={0,10000,20000},
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries},
%ylabel style={yshift=-0.25in},
%ylabel={Frequency},
legend style={at={(0.5,1.43)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\footnotesize,nodes={scale=0.9, transform shape}},
legend columns=5,
grid=major
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=red,line width=1.6pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0001 0\\
0.0001148153621496883 0\\
0.00013182567385564074 0\\
0.00015135612484362088 0\\
0.00017378008287493763 0\\
0.00019952623149688788 0\\
0.00022908676527677723 0\\
0.00026302679918953814 0\\
0.0003019951720402016 0\\
0.0003467368504525317 0\\
0.00039810717055349735 1\\
0.0004570881896148752 0\\
0.0005248074602497723 1\\
0.0006025595860743581 1\\
0.0006918309709189362 1\\
0.0007943282347242813 1\\
0.0009120108393559096 2\\
0.0010471285480508996 5\\
0.001202264434617413 4\\
0.0013803842646028838 8\\
0.001584893192461114 13\\
0.0018197008586099826 13\\
0.0020892961308540386 13\\
0.00239883291901949 22\\
0.002754228703338166 20\\
0.0031622776601683794 29\\
0.003630780547701014 46\\
0.004168693834703355 46\\
0.00478630092322638 44\\
0.005495408738576248 57\\
0.00630957344480193 69\\
0.007244359600749898 58\\
0.008317637711026709 91\\
0.009549925860214359 109\\
0.01096478196143185 132\\
0.012589254117941675 115\\
0.01445439770745928 157\\
0.016595869074375595 177\\
0.019054607179632463 154\\
0.02187761623949552 196\\
0.025118864315095794 237\\
0.028840315031266057 214\\
0.03311311214825911 274\\
0.038018939632056124 255\\
0.04365158322401656 284\\
0.0501187233627272 295\\
0.057543993733715666 307\\
0.06606934480075957 324\\
0.07585775750291836 307\\
0.08709635899560805 336\\
0.1 363\\
0.1148153621496883 353\\
0.13182567385564073 339\\
0.1513561248436207 327\\
0.17378008287493746 276\\
0.1995262314968879 267\\
0.22908676527677724 276\\
0.26302679918953814 274\\
0.3019951720402016 262\\
0.34673685045253166 239\\
0.3981071705534969 212\\
0.4570881896148747 172\\
0.5248074602497723 170\\
0.6025595860743574 154\\
0.6918309709189363 135\\
0.7943282347242814 133\\
0.9120108393559097 121\\
1.0471285480508985 108\\
1.2022644346174132 110\\
1.3803842646028839 92\\
1.584893192461114 89\\
1.8197008586099825 74\\
2.089296130854041 71\\
2.39883291901949 65\\
2.754228703338163 56\\
3.1622776601683795 54\\
3.63078054770101 26\\
4.168693834703355 33\\
4.7863009232263805 39\\
5.4954087385762485 20\\
6.30957344480193 30\\
7.244359600749891 30\\
8.317637711026709 21\\
9.54992586021435 38\\
10.964781961431852 36\\
12.589254117941662 23\\
14.45439770745928 28\\
16.595869074375596 41\\
19.054607179632445 29\\
21.87761623949552 28\\
25.11886431509577 52\\
28.84031503126606 32\\
33.11311214825908 30\\
38.018939632056124 12\\
43.65158322401656 17\\
50.11872336272725 15\\
57.543993733715666 5\\
66.06934480075951 1\\
75.85775750291836 6\\
87.09635899560796 1\\
};
\addlegendentry{(P).UC}

\addplot [color=green,line width=1.6pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0001 0\\
0.0001148153621496883 0\\
0.00013182567385564074 0\\
0.00015135612484362088 0\\
0.00017378008287493763 0\\
0.00019952623149688788 0\\
0.00022908676527677723 0\\
0.00026302679918953814 0\\
0.0003019951720402016 0\\
0.0003467368504525317 0\\
0.00039810717055349735 0\\
0.0004570881896148752 0\\
0.0005248074602497723 2\\
0.0006025595860743581 1\\
0.0006918309709189362 2\\
0.0007943282347242813 1\\
0.0009120108393559096 3\\
0.0010471285480508996 3\\
0.001202264434617413 3\\
0.0013803842646028838 7\\
0.001584893192461114 7\\
0.0018197008586099826 6\\
0.0020892961308540386 11\\
0.00239883291901949 26\\
0.002754228703338166 24\\
0.0031622776601683794 36\\
0.003630780547701014 45\\
0.004168693834703355 43\\
0.00478630092322638 44\\
0.005495408738576248 72\\
0.00630957344480193 86\\
0.007244359600749898 113\\
0.008317637711026709 128\\
0.009549925860214359 149\\
0.01096478196143185 158\\
0.012589254117941675 171\\
0.01445439770745928 196\\
0.016595869074375595 177\\
0.019054607179632463 196\\
0.02187761623949552 247\\
0.025118864315095794 250\\
0.028840315031266057 269\\
0.03311311214825911 297\\
0.038018939632056124 293\\
0.04365158322401656 353\\
0.0501187233627272 335\\
0.057543993733715666 346\\
0.06606934480075957 341\\
0.07585775750291836 334\\
0.08709635899560805 291\\
0.1 303\\
0.1148153621496883 290\\
0.13182567385564073 250\\
0.1513561248436207 272\\
0.17378008287493746 223\\
0.1995262314968879 255\\
0.22908676527677724 240\\
0.26302679918953814 230\\
0.3019951720402016 195\\
0.34673685045253166 201\\
0.3981071705534969 184\\
0.4570881896148747 154\\
0.5248074602497723 145\\
0.6025595860743574 172\\
0.6918309709189363 119\\
0.7943282347242814 117\\
0.9120108393559097 104\\
1.0471285480508985 93\\
1.2022644346174132 90\\
1.3803842646028839 106\\
1.584893192461114 64\\
1.8197008586099825 69\\
2.089296130854041 70\\
2.39883291901949 48\\
2.754228703338163 53\\
3.1622776601683795 69\\
3.63078054770101 49\\
4.168693834703355 45\\
4.7863009232263805 35\\
5.4954087385762485 28\\
6.30957344480193 42\\
7.244359600749891 34\\
8.317637711026709 50\\
9.54992586021435 37\\
10.964781961431852 34\\
12.589254117941662 31\\
14.45439770745928 35\\
16.595869074375596 40\\
19.054607179632445 25\\
21.87761623949552 28\\
25.11886431509577 23\\
28.84031503126606 20\\
33.11311214825908 16\\
38.018939632056124 11\\
43.65158322401656 10\\
50.11872336272725 4\\
57.543993733715666 5\\
66.06934480075951 0\\
75.85775750291836 4\\
87.09635899560796 2\\
};
\addlegendentry{(P).C}

\addplot [color=blue,line width=1.6pt, dashed, mark options={solid, red}]
  table[row sep=crcr]{%
0.0001 0\\
0.0001148153621496883 0\\
0.00013182567385564074 0\\
0.00015135612484362088 0\\
0.00017378008287493763 0\\
0.00019952623149688788 0\\
0.00022908676527677723 0\\
0.00026302679918953814 0\\
0.0003019951720402016 0\\
0.0003467368504525317 0\\
0.00039810717055349735 0\\
0.0004570881896148752 0\\
0.0005248074602497723 2\\
0.0006025595860743581 1\\
0.0006918309709189362 2\\
0.0007943282347242813 1\\
0.0009120108393559096 4\\
0.0010471285480508996 3\\
0.001202264434617413 3\\
0.0013803842646028838 8\\
0.001584893192461114 7\\
0.0018197008586099826 7\\
0.0020892961308540386 12\\
0.00239883291901949 27\\
0.002754228703338166 26\\
0.0031622776601683794 36\\
0.003630780547701014 47\\
0.004168693834703355 45\\
0.00478630092322638 49\\
0.005495408738576248 75\\
0.00630957344480193 88\\
0.007244359600749898 121\\
0.008317637711026709 134\\
0.009549925860214359 151\\
0.01096478196143185 162\\
0.012589254117941675 172\\
0.01445439770745928 201\\
0.016595869074375595 185\\
0.019054607179632463 195\\
0.02187761623949552 245\\
0.025118864315095794 255\\
0.028840315031266057 264\\
0.03311311214825911 308\\
0.038018939632056124 299\\
0.04365158322401656 357\\
0.0501187233627272 334\\
0.057543993733715666 359\\
0.06606934480075957 351\\
0.07585775750291836 332\\
0.08709635899560805 312\\
0.1 293\\
0.1148153621496883 292\\
0.13182567385564073 257\\
0.1513561248436207 272\\
0.17378008287493746 242\\
0.1995262314968879 256\\
0.22908676527677724 238\\
0.26302679918953814 218\\
0.3019951720402016 194\\
0.34673685045253166 193\\
0.3981071705534969 191\\
0.4570881896148747 162\\
0.5248074602497723 145\\
0.6025595860743574 162\\
0.6918309709189363 111\\
0.7943282347242814 105\\
0.9120108393559097 107\\
1.0471285480508985 82\\
1.2022644346174132 94\\
1.3803842646028839 104\\
1.584893192461114 68\\
1.8197008586099825 62\\
2.089296130854041 69\\
2.39883291901949 58\\
2.754228703338163 51\\
3.1622776601683795 65\\
3.63078054770101 36\\
4.168693834703355 33\\
4.7863009232263805 28\\
5.4954087385762485 25\\
6.30957344480193 38\\
7.244359600749891 26\\
8.317637711026709 33\\
9.54992586021435 34\\
10.964781961431852 29\\
12.589254117941662 31\\
14.45439770745928 29\\
16.595869074375596 41\\
19.054607179632445 26\\
21.87761623949552 29\\
25.11886431509577 18\\
28.84031503126606 17\\
33.11311214825908 18\\
38.018939632056124 10\\
43.65158322401656 11\\
50.11872336272725 6\\
57.543993733715666 4\\
66.06934480075951 0\\
75.85775750291836 7\\
87.09635899560796 1\\
};
\addlegendentry{(P).H}


\legend{}

\end{axis}

%\end{tikzpicture}%

==> figs/real_test_3v_e.tex <==
\begin{tikzpicture}

\begin{axis}[%
xmode=log,
width=0.4\columnwidth,
height=0.25\columnwidth,
at={(0in,0.389in)},
scale only axis,
xmin=1e-5,
xmax=100,
xlabel style={font=\color{white!15!black}},
xlabel={Triangulation error (m)},
%xtick={1e-15,1e-10,1e-5,1e-0},
title={$m=3$},
ymin=0,
ymax=400,
ymode=normal,
yminorticks=true,
%ytick={0,10000,20000},
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries},
%ylabel style={yshift=-0.25in},
ylabel={Frequency},
legend style={at={(0.5,1.33)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\footnotesize,nodes={scale=0.9, transform shape}},
legend columns=5
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=red,line width=1.6pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0001 0\\
0.0001148153621496883 0\\
0.00013182567385564074 0\\
0.00015135612484362088 0\\
0.00017378008287493763 0\\
0.00019952623149688788 0\\
0.00022908676527677723 0\\
0.00026302679918953814 0\\
0.0003019951720402016 0\\
0.0003467368504525317 0\\
0.00039810717055349735 1\\
0.0004570881896148752 0\\
0.0005248074602497723 0\\
0.0006025595860743581 0\\
0.0006918309709189362 0\\
0.0007943282347242813 0\\
0.0009120108393559096 0\\
0.0010471285480508996 2\\
0.001202264434617413 0\\
0.0013803842646028838 6\\
0.001584893192461114 6\\
0.0018197008586099826 5\\
0.0020892961308540386 4\\
0.00239883291901949 9\\
0.002754228703338166 10\\
0.0031622776601683794 10\\
0.003630780547701014 23\\
0.004168693834703355 15\\
0.00478630092322638 24\\
0.005495408738576248 32\\
0.00630957344480193 36\\
0.007244359600749898 30\\
0.008317637711026709 44\\
0.009549925860214359 52\\
0.01096478196143185 54\\
0.012589254117941675 62\\
0.01445439770745928 75\\
0.016595869074375595 99\\
0.019054607179632463 79\\
0.02187761623949552 112\\
0.025118864315095794 138\\
0.028840315031266057 118\\
0.03311311214825911 167\\
0.038018939632056124 150\\
0.04365158322401656 176\\
0.0501187233627272 173\\
0.057543993733715666 165\\
0.06606934480075957 216\\
0.07585775750291836 198\\
0.08709635899560805 197\\
0.1 224\\
0.1148153621496883 211\\
0.13182567385564073 202\\
0.1513561248436207 183\\
0.17378008287493746 159\\
0.1995262314968879 145\\
0.22908676527677724 157\\
0.26302679918953814 139\\
0.3019951720402016 135\\
0.34673685045253166 114\\
0.3981071705534969 85\\
0.4570881896148747 74\\
0.5248074602497723 72\\
0.6025595860743574 67\\
0.6918309709189363 61\\
0.7943282347242814 57\\
0.9120108393559097 43\\
1.0471285480508985 41\\
1.2022644346174132 29\\
1.3803842646028839 26\\
1.584893192461114 22\\
1.8197008586099825 16\\
2.089296130854041 17\\
2.39883291901949 21\\
2.754228703338163 15\\
3.1622776601683795 14\\
3.63078054770101 5\\
4.168693834703355 7\\
4.7863009232263805 5\\
5.4954087385762485 1\\
6.30957344480193 5\\
7.244359600749891 3\\
8.317637711026709 3\\
9.54992586021435 8\\
10.964781961431852 6\\
12.589254117941662 7\\
14.45439770745928 12\\
16.595869074375596 18\\
19.054607179632445 21\\
21.87761623949552 20\\
25.11886431509577 47\\
28.84031503126606 21\\
33.11311214825908 24\\
38.018939632056124 2\\
43.65158322401656 2\\
50.11872336272725 9\\
57.543993733715666 1\\
66.06934480075951 0\\
75.85775750291836 3\\
87.09635899560796 0\\
};
\addlegendentry{(P).UC}

\addplot [color=green,line width=1.6pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0001 0\\
0.0001148153621496883 0\\
0.00013182567385564074 0\\
0.00015135612484362088 0\\
0.00017378008287493763 0\\
0.00019952623149688788 0\\
0.00022908676527677723 0\\
0.00026302679918953814 0\\
0.0003019951720402016 0\\
0.0003467368504525317 0\\
0.00039810717055349735 0\\
0.0004570881896148752 0\\
0.0005248074602497723 1\\
0.0006025595860743581 0\\
0.0006918309709189362 1\\
0.0007943282347242813 1\\
0.0009120108393559096 1\\
0.0010471285480508996 0\\
0.001202264434617413 1\\
0.0013803842646028838 3\\
0.001584893192461114 2\\
0.0018197008586099826 5\\
0.0020892961308540386 5\\
0.00239883291901949 10\\
0.002754228703338166 13\\
0.0031622776601683794 15\\
0.003630780547701014 24\\
0.004168693834703355 26\\
0.00478630092322638 32\\
0.005495408738576248 39\\
0.00630957344480193 62\\
0.007244359600749898 77\\
0.008317637711026709 80\\
0.009549925860214359 83\\
0.01096478196143185 103\\
0.012589254117941675 121\\
0.01445439770745928 129\\
0.016595869074375595 104\\
0.019054607179632463 128\\
0.02187761623949552 172\\
0.025118864315095794 169\\
0.028840315031266057 190\\
0.03311311214825911 211\\
0.038018939632056124 178\\
0.04365158322401656 224\\
0.0501187233627272 223\\
0.057543993733715666 203\\
0.06606934480075957 209\\
0.07585775750291836 197\\
0.08709635899560805 167\\
0.1 148\\
0.1148153621496883 159\\
0.13182567385564073 141\\
0.1513561248436207 139\\
0.17378008287493746 109\\
0.1995262314968879 124\\
0.22908676527677724 119\\
0.26302679918953814 93\\
0.3019951720402016 80\\
0.34673685045253166 78\\
0.3981071705534969 78\\
0.4570881896148747 63\\
0.5248074602497723 62\\
0.6025595860743574 63\\
0.6918309709189363 33\\
0.7943282347242814 40\\
0.9120108393559097 18\\
1.0471285480508985 20\\
1.2022644346174132 18\\
1.3803842646028839 26\\
1.584893192461114 18\\
1.8197008586099825 11\\
2.089296130854041 11\\
2.39883291901949 4\\
2.754228703338163 10\\
3.1622776601683795 12\\
3.63078054770101 6\\
4.168693834703355 7\\
4.7863009232263805 2\\
5.4954087385762485 1\\
6.30957344480193 6\\
7.244359600749891 1\\
8.317637711026709 3\\
9.54992586021435 5\\
10.964781961431852 5\\
12.589254117941662 11\\
14.45439770745928 15\\
16.595869074375596 20\\
19.054607179632445 13\\
21.87761623949552 21\\
25.11886431509577 15\\
28.84031503126606 11\\
33.11311214825908 13\\
38.018939632056124 6\\
43.65158322401656 1\\
50.11872336272725 1\\
57.543993733715666 0\\
66.06934480075951 0\\
75.85775750291836 0\\
87.09635899560796 0\\
};
\addlegendentry{(P).C}

\addplot [color=blue,line width=1.6pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0001 0\\
0.0001148153621496883 0\\
0.00013182567385564074 0\\
0.00015135612484362088 0\\
0.00017378008287493763 0\\
0.00019952623149688788 0\\
0.00022908676527677723 0\\
0.00026302679918953814 0\\
0.0003019951720402016 0\\
0.0003467368504525317 0\\
0.00039810717055349735 0\\
0.0004570881896148752 0\\
0.0005248074602497723 1\\
0.0006025595860743581 0\\
0.0006918309709189362 1\\
0.0007943282347242813 1\\
0.0009120108393559096 1\\
0.0010471285480508996 0\\
0.001202264434617413 1\\
0.0013803842646028838 3\\
0.001584893192461114 2\\
0.0018197008586099826 5\\
0.0020892961308540386 6\\
0.00239883291901949 10\\
0.002754228703338166 13\\
0.0031622776601683794 15\\
0.003630780547701014 25\\
0.004168693834703355 27\\
0.00478630092322638 34\\
0.005495408738576248 40\\
0.00630957344480193 63\\
0.007244359600749898 81\\
0.008317637711026709 83\\
0.009549925860214359 84\\
0.01096478196143185 104\\
0.012589254117941675 122\\
0.01445439770745928 128\\
0.016595869074375595 107\\
0.019054607179632463 126\\
0.02187761623949552 173\\
0.025118864315095794 169\\
0.028840315031266057 182\\
0.03311311214825911 209\\
0.038018939632056124 176\\
0.04365158322401656 226\\
0.0501187233627272 219\\
0.057543993733715666 204\\
0.06606934480075957 209\\
0.07585775750291836 202\\
0.08709635899560805 175\\
0.1 147\\
0.1148153621496883 157\\
0.13182567385564073 146\\
0.1513561248436207 141\\
0.17378008287493746 112\\
0.1995262314968879 126\\
0.22908676527677724 122\\
0.26302679918953814 90\\
0.3019951720402016 80\\
0.34673685045253166 72\\
0.3981071705534969 74\\
0.4570881896148747 65\\
0.5248074602497723 56\\
0.6025595860743574 54\\
0.6918309709189363 31\\
0.7943282347242814 38\\
0.9120108393559097 18\\
1.0471285480508985 22\\
1.2022644346174132 20\\
1.3803842646028839 22\\
1.584893192461114 20\\
1.8197008586099825 10\\
2.089296130854041 12\\
2.39883291901949 8\\
2.754228703338163 12\\
3.1622776601683795 12\\
3.63078054770101 3\\
4.168693834703355 5\\
4.7863009232263805 3\\
5.4954087385762485 1\\
6.30957344480193 6\\
7.244359600749891 1\\
8.317637711026709 3\\
9.54992586021435 5\\
10.964781961431852 3\\
12.589254117941662 10\\
14.45439770745928 13\\
16.595869074375596 18\\
19.054607179632445 15\\
21.87761623949552 21\\
25.11886431509577 13\\
28.84031503126606 8\\
33.11311214825908 13\\
38.018939632056124 6\\
43.65158322401656 2\\
50.11872336272725 2\\
57.543993733715666 1\\
66.06934480075951 0\\
75.85775750291836 2\\
87.09635899560796 0\\
};
\addlegendentry{(P).H}


%\legend{}

\end{axis}

\end{tikzpicture}%
